Condensation de tachyon dans le syst\`eme brane-antibrane

In superstring theory of type II, the separated brane-antibrane pair admits a bi-fundamental tachyon in its open string spectrum, for any separation less than the critical distance. The dynamics of this system would be described by the Garousi's effective action for any non-zero separation. Our study shows however that the domain of validity of this action only includes space-like tachyon condensation. Previous studies led by Bagchi and Sen showed that, in a partial sub-critical domain, exists a conformal field theory (CFT), which describes a dynamical condensation at static distance, called rolling tachyon. We show that this CFT actually exists on the whole tachyonic domain. Thanks to this demonstration, we prove that the domain of validity of Garousi's action excludes time-dependent tachyon condensation, and we justify the computation of the partition fonction along the rolling tachyon on the whole sub-critical domain. Using a method proposed by Kutasov and Niarchos, we determine a quadratic effective action for the tachyon and distance fields, at least valid in the whole tachyonic domain around the rolling tachyon solution. In addition, we studied the non linear sigma model of perturbative deformations along the rolling tachyon CFT. The beta-function of the renormalization group, that we obtained, are in good agreement with the equations of movement derived from the proposed quadratic effective action. This stands as an independent confirmation of its expression.

==> introduction_final.tex <==

\chapter{Motivations et plan de th\`ese}
\label{chap:mot}

\input{chap_motivation}

\chapter{G\'en\'eralit\'es~: Th\'eorie des cordes et th\'eories des champs conformes de surface}
\label{chap:TDC_CFT}

\input{chap_generalite1}


\chapter{G\'en\'eralit\'es~: th\'eories effectives et mod\`ele sigma}
\label{chap:TEC_sigma}

\input{chap_generalite2}


\chapter{G\'en\'eralit\'es~: Condensation de tachyon de cordes ouvertes}
\label{chap:cond_tach}

\input{chap_generalite3}

==> part_conclusion_ex.tex <==
\part{Conclusion et perspectives}
\label{part:conclu}


Au cours de cette thèse, nous avons démontré que le tachyon roulant du secteur interbranaire (anti-diagonal) $\sigma^\pm \in U(2)$ dans le système d'une brane et d'une antibrane parallèles et séparées en théorie de type IIA ou IIB, est une solution des \'equations du mouvement de la théorie des champs de cordes dans l'\emph{ensemble} du domaine tachyonique $\ell<\ell_c$ avec $\ell_c = \pi\sqrt{2\alpha'}$. Le modèle sigma incluant l'opérateur de vertex de ce tachyon roulant constitue ainsi une théorie des champs conforme. Nous nous sommes intéressés aussi au modèle bosonique correspondant qui non seulement admet un tachyon interbranaire dans son spectre de corde ouverte mais contient aussi des tachyons hébergés sur chaque brane, \cad dans les secteurs diagonaux $\sigma^{0,3} \in U(2)$. 

Dans le premier cas, nous avons montré que les résonances entre les opérateurs de tachyons roulants $\sigma^\pm \otimes \psi^\pm e^{\sqrt{1/2-r^2} X^0 \pm ir\wt X}$ avec $r=\ell/2\pi$ et l'opérateur $\sigma^0 \otimes e^{2 n \sqrt{1/2-r^2}X^0}$ n'engageaient aucune divergence logarithmique à l'ordre 2 et 4 dans les tachyons, \cad pour tout $r<\sqrt{17}/6$. En identifiant le mécanisme d'annulation de ces divergences au rôle de la supersymétrie, nous en avons déduit que cela devait s'appliquer à tout ordre et à toute distance. Nous avons vu que les divergences logarithmiques étaient la cause de la perte de marginalité en contribuant à l'expression des fonctions bêta des couplages associés aux opérateurs produit par résonance. L'absence des divergences logarithmiques nous a ainsi permis de conclure à la marginalité exacte du modèle de tachyon roulant dans le système brane-antibrane. Nous nous attendions à ce comportement par absence de raisons \emph{physiques} justifiant le contraire. 

Dans le second cas, nous avons vu en revanche que les résonances entre les tachyons roulants $\sigma^\pm \otimes e^{\sqrt{1-r^2} X^0 \pm ir\wt X}$ et l'opérateur $\sigma^0 \otimes e^{2 n \sqrt{1-r^2}X^0}$ faisaient intervenir des divergences logarithmiques -- non supprimées -- au moins à l'ordre 2 pour tout $r>r_c/\sqrt 2$. Nous en avons déduit que les contributions correspondantes dans les fonctions bêta du champ de tachyon du secteur $\sigma^0$ mettaient en valeur l'existence d'un couplage \emph{physique} non nul dans l'action effective du système entre ce tachyon et celui du secteur interbranaire. 

Ainsi, dans un cas nous obtenons une suppression des divergences logarithmiques gr\^ace à la supersymétrie, et dans l'autre cas, il n'existe aucune supersymétrie et ces divergences ne s'annulent pas. Dans le premier il n'y a aucune raison physique qui justifierait la présence de divergences logarithmiques à cause de la supersymétrie et de la projection GSO qui supprime le mode tachyonique des secteurs diagonaux. Mais dans le second, puisque le tachyon du secteur $\sigma^0$ est une excitation physique dans le modèle bosonique, nous avons une raison \emph{physique} pour expliquer la présence de divergences logarithmiques. \\

Dans le système brane-antibrane, nous avons aussi mis en valeur l'existence de termes de contact. Ces derniers apparaissent naturellement en exprimant l'action de surface de corde de façon manifestement supersymétrique dans le super-espace en introduisant des fermions de bord, puis en décomposant cette action et en intégrant sur les variables de Grassmann.  Nous avons montré que ces termes de contact jouaient le rôle de contretermes et permettaient de supprimer un grand nombre de divergences en puissance du cut-off UV $\varepsilon$ dans les amplitudes, ou au moins dans la fonction de partition sur le disque. Ce comportement relève d'une théorie manifestement supersymétrique. Or les résultats précédents ont montré que les divergences en puissance n'étaient pas \emph{toutes} supprimées et qu'il restait des divergences résiduelles. Nous avons identifiées qu'elles étaient \^otables par des termes de contact d'ordre supérieur et nous avons donc proposé de corriger l'action supersymétrique des fermions de bord en conséquence, par l'ajout de termes d'interaction à 4 points et plus. 

A distance $\ell<\ell_c$ le nombre de termes divergents à tout ordre est fini. En effet, à distance $\ell$ pour une fonction à $2N$-points des tachyons la "divergence" résiduelle est du type $\varepsilon^{4N^2(1/2 -r^2)-1} \oint e^{2 N \sqrt{1/2-r^2}X^0}$ pour tout $N <1/(2-4r^2)$. Ainsi, le nombre de contretermes à ajouter dans l'action est fini et la théorie renormalisable. Puisqu'il s'agit de divergences de puissance, la théorie reste en outre exactement marginale. Cependant dans la limite $ r\to r_c$ le nombre de divergences résiduelles tend vers l'infini. Ainsi la limite $r\to r_c^-$ ne définit pas une théorie renormalisable. La valeur $r_c$ est, aussi en ce sens, une distance critique. Nous identifions ce comportement à la perte de marginalité du tachyon roulant en $r=r_c$ à cause d'une résonance non nulle avec le champ de distance $\sigma^3 \otimes D\wt {\mathbb X}$. Cela pourrait \^etre d\^u \`a la transition d'une théorie interactive $c=2$ à une théorie interactive $c=1$ par comparaison au comportement des théories Liouville dans la limite $c\to 1$. \\


Notre étude a porté ensuite sur le groupe de renormalisation du modèle sigma perturbé autour de la déformation marginale du tachyon roulant dans le cas bosonique et dans le cas brane-antibrane. 
D'abord en théorie bosonique, nous avons inséré sur le bord la déformation correspondante à une perturbation de distance $\delta r(X^a)$ et nous avons supposé que le tachyon lui-même était une perturbation $\lambda^\pm(X^a)$. Pour étudier le groupe de renormalisation de ces perturbations et obtenir des contraintes physiques sur leur dynamique respective, nous avons développé ces fonctions des champs $X$ en décomposant ces derniers en mode zéro et modes d'oscillations $X=x+\hat X$. Nous obtenions alors des perturbations \emph{relevantes} autour des déformations marginales. De ce fait, les fonctions b\^eta obtenues pour les couplages $\delta r(x)$ et $\lambda^\pm(x)$ ne pouvaient recevoir de contributions que via des résonances, donc des termes logarithmiques et universels, \cad indépendant des schémas de renormalisation. Nous avons justifié dans cette mesure l'interprétation de ces fonctions b\^eta en tant qu'équations du mouvement. Leur expression obtenue est non triviale et prend son origine dans l'existence d'une solution de type S-brane complète à l'ordre quadratique. En l'état, ces équations ne permettent pas d'exprimer une action effective dont elles dérivent, à moins de redéfinir les champs ou les fonctions b\^eta par des termes constants ou proportionnels à d'autres fonctions b\^eta, ce que nous voyons concrètement dans la section~\refcc{sec:act_eff_kut}.

Dans le modèle brane-antibrane, nous avons exprimé une théorie équivalente, manifestement supersymétrique sur le super-espace de la surface de corde, puisque nous avions vu l'importance que revêtaient les termes de contact dans l'extraction des divergences. Les perturbations ont donc été exprimées dans le super-espace, et autour des déformations marginales, par $\delta r({\mathbb X}^a)$ et $\lambda^\pm({\mathbb X}^a)$. Après décomposition des superchamps, \cad développement par $X = x + \hat X$ et intégration des champs auxiliaires, nous avons obtenu divers termes de contact et des expressions non triviales des opérateurs \emph{relevants} couplés aux champs et leurs dérivés. Nous avons obtenu la suppression d’un certain nombre de divergences logarithmiques gr\^ace aux termes de contact. Néanmoins à partir de termes logarithmiques résiduels nous avons de nouveau calculé des fonctions bêta non triviales pour les couplages $\delta r(x)$ et $\lambda^\pm(x)$ puis des expressions pour les équations du mouvement correspondantes. Leurs expressions sont très semblables à celles du modèle bosonique, indiquant que la physique entre ces deux systèmes est très similaire, sauf dans le domaine $\ell>\ell_c/\sqrt 2$ car dans le modèle bosonique le couplage du tachyon interbranaire au tachyon du secteur $\sigma^{0,3}$ y est effectif. 

De m\^eme que dans le cas bosonique, les formules na\"ives des équations du mouvement obtenues à partir des fonctions b\^eta ne sont pas compatibles avec une action effective. Toutefois, la comparaison de ces équations à celles dérivées de l'action effective quadratique obtenue dans la section~\refcc{sec:act_eff_kut} associée à une analyse attentive des fonctions b\^eta, montre qu'en ajoutant à leurs expressions des termes proportionnels aux fonctions b\^eta et en redéfinissant certains champs, nous pouvons en réalité en dériver des équations de mouvement compatibles avec une action effective.  \\ 


Dans la section~\refcc{sec:act_eff_kut} nous avons utilisé la méthode proposée par Kutasov et Niarchos afin de calculer exactement l'action effective à l'ordre quadratique. Ils proposent de contraindre un ansatz d'action effective à l'ordre des dérivées premières -- ce qui est justifié le long de tachyons de type quasi-homogènes, \cad tant que leurs oscillations spatiales sont de grandes longueurs d'onde -- en imposant que ses équations du mouvement admettent la solution de S-brane complète. Cela permet de réduire considérablement, au moins dans leur modèle, le nombre de degrés de liberté de l'ansatz –- en l'occurence à un par ordre dans le tachyon.  Par comparaison à l'expression de la fonction de partition sur le disque, le long de la solution de demi S-brane, en utilisant l'identité $S_{\text{on-shell}}=Z$ l'ansatz est alors complètement contraint et l'action effective totalement déterminée. L'action obtenue par cette méthode est au moins valable autour de cette solution.

Nous avons cependant montré que dans le système brane-antibrane s\'epar\'e, il n'est pas possible de déterminer entièrement un ansatz d'action par cette méthode. En effet, la forme spécifique de la solution de S-brane complète dans ce cas précis ne permet d'exprimer qu'un système d'équations sous-déterminé pour l'ansatz. Par conséquent, nous ne pouvons pas réduire son nombre de degrés de liberté aussi significativement que dans le système étudié par Kutasov et Niarchos. Alors, l'action effective ne peut pas \^etre totalement déterminée par la formule $S_{\text{on-shell}}=Z$. Néanmoins, nous avons la possibilité de calculer exactement une action à l'ordre quartique dans le tachyon. En effet, le nombre de degré de liberté par ordre dans le tachyon étant alors réduit à un, nous pouvons les contraindre par la formule ci-dessus et obtenir une expression quartique pour l'action effective du système brane-antibrane. \\

Par ailleurs, nous avons exprimé la fonction de partition sur le disque le long du tachyon roulant. Nous avons développé une méthode diagrammatique afin de traiter analytiquement les intégrandes et réduire l'intégrale de chemin définie dans le super-espace à une intégrale de chemin définie sur le disque. L'expression finale que nous obtenons pour tout $r<r_c$ est telle que le calcul analytique de l'intégrale à tout ordre est hors de portée. Nous avons cependant pu calculer la densit\'e de fonction de partition, not\'ee $Z'$, à l'ordre 8 dans les tachyons pour la distance $r=r_c/\sqrt 2$. Nous espérions obtenir une expression connue du développement, mais les résultats ordre par ordre semblent se complexifier à mesure que l'ordre augmente. Nous ne reconnaissons aucune série connue dans sa formule~:

\begin{multline}
Z'(x^0) = 1 - \lambda^+\lambda^- \frac{e^{x^0}}{\pi} + \frac{\parent{\lambda^+\lambda^-}^2}{\pi^2} e^{2 x^0}\parent{1 -\frac{\pi^2}{6}} -  \frac{\parent{\lambda^+\lambda^-}^3}{\pi^3} e^{3 x^0} \parent{1 - \frac{128}{3 \pi^2}} \\+ \frac{\parent{\lambda^+\lambda^-}^4}{\pi^4} e^{4 x^0} \parent{1-\frac{55}{12}+\frac{143}{9 \pi ^2}+\frac{13 \pi ^2}{30}+\frac{\pi ^4}{70}+\frac{175}{27}+\frac{1001}{162 \pi ^2}+\frac{\pi ^2}{15}} \ldots 
\end{multline}

Nous avons aussi pu calculer exactement l'ordre quadratique ce qui nous a permis de déterminer au moins une action effective à l'ordre quadratique par la méthode présentée ci-dessus. L'expression de l'action effective à l'ordre quadratique pour le tachyon et la distance est~:

\begin{align}\label{eq:act_eff_conclu}
&{\mathcal L} = 2\Bigg[1 + \frac{\pi^2}{2}\partial_a r \partial^a r  + \frac{1}{2 \sqrt{1 - 2r^2}}\parent{\partial_a T\partial^a T^*-\parent{\frac{1}{2}-r^2} \module{T}^2} + \ldots \Bigg] 
\end{align}

Cette expression comme celle de l'action obtenue par Kutasov et Niarchos n'est valable que le long de la solution de référence. Donc son domaine de validité concerne les perturbations des champs autour du tachyon roulant à distance constante. Cette expression est nettement différente de celle correspondant au développement quadratique de l'action de Garousi. Ce qui n’est pas surprenant, puisque nous argumentons en introduction que l'action de Garousi n'est \apriori valable que pour des tachyons de genre espace, \cad non dynamique. En outre, l'action de Garousi n'admet pas de solution de tachyon roulant à distance constante comme nous l’avons démontré. 

Comme nous le disons plus haut, la dérivation des équations du mouvement à partir de~\refe{eq:act_eff_conclu} a montré après une analyse attentive que les équations obtenues par le biais du groupe de renormalisation étaient compatibles avec cette action. L'absence à premier abord d'un terme d'interaction entre la dérivée du tachyon et la dérivée du champ de distance rendait la correspondance impossible. Toutefois nous avons pu identifier ce terme à une contribution proportionnelle à la fonction bêta de $\Delta \lambda^\pm$ à l'ordre quadratique. Or nous savons que les fonctions bêta sont soumises à cette ambiguïté~\cite{Tseytlin:1986zz} lorsque nous voulons les interpréter en tant qu'équations du mouvement. La compatibilité entre ces deux développements semble donc plutôt correcte. \\

Nous conclurons cette étude en présentant les similitudes que revêtent les modèles de tachyon du secteur interbranaire et les modèles de Kondo bosoniques -- et par conséquent aussi supersymétriques. Le modèle de Kondo est défini par l'hamiltonien suivant~\cite{LeClair:1997sd} sur le demi-plan complexe avec $z=x+iy$~:

\begin{equation}\label{eq:kondo_hamil}
H_K = \frac{1}{2} \int_{-\infty}^{+\infty} \di x ~ \parent{ \parent{\partial_x \phi}^2 + \parent{\partial_y \phi}^2 } + \omega_0 \parent{S^+ e^{i \beta \phi(0,y)} + S^- e^{-i \beta \phi(0,y)}}
\end{equation}

Les matrices $S^\pm$ agissent dans une représentation de spin $j/2$ de $SU(2)_q$ avec $q=e^{i\pi \beta^2}$. Voir~\refe{eq:algebre_q} plus loin. Par comparaison, le lagrangien du modèle de tachyon interbranaire constant est donné par~:

\begin{equation}\label{eq:kondo_lag}
S = \frac{1}{2 \pi} \int \di{x} \di{y} ~ \parent{ \parent{\partial_x \phi}^2 + \parent{\partial_y \phi}^2 } + \oint \di{y} ~ \parent{ \lambda^+ \sigma^+ e^{i \beta \phi(0,y)} + \lambda^- \sigma^- e^{-i \beta \phi(0,y)}}
\end{equation}  

où $\sigma^\pm$ appartiennent à la représentation $1/2$ de $SU(2)$ en fait équivalente à une représentation $1/2$ de $SU(2)_q$. Nous voyons donc par transformation de Legendre de~\refe{eq:kondo_lag} que la correspondance est ici donnée par $\omega_0 = - \lambda^\pm$ et $S^\pm = \sigma^\pm$. La relation du modèle de Kondo au modèle de sine-Gordon de bord (BSG) est bien connue -- voir par exemple~\cite{Fendley:1995kj}. En l’occurrence, les fonctions de partition respectives vérifient certaines relations comme nous voyons un peu plus bas dans la formule~\refe{eq:partition_kondo_BSG}. En outre, le modèle Kondo est intégrable à condition que les matrices $S^\pm$ appartiennent bien à la représentation $j/2$ de $SU(2)_q$ et vérifient l'algèbre~:

\begin{align}\label{eq:algebre_q}
\comm{S^+}{S^-} = \frac{q^{S_z}-q^{-S_z}}{q-q^{-1}} \qquad \comm{S_z}{S^\pm}=\pm 2 S^\pm
\end{align}

qui est effectivement la même que $SU(2)$ le long d'une représentation $1/2$. Le modèle a deux régimes autour de la limite de Toulouse $\beta\to 1/\sqrt 2$ qui, par comparaison à l'étude du tachyon roulant dans le modèle bosonique, est celle à partir de laquelle le couplage aux tachyons du secteur $\sigma^0$ est effectif. Pour $\beta< 1/\sqrt 2$ on parle de régime attractif et pour $1>\beta> 1/\sqrt 2$ de régime répulsif. Dans ce dernier régime la fonction de partition sur le disque a des pôles pour tout $\beta =\sqrt{ (1+2n )/(2+2n)} $. Dans le premier la fonction de partition est analytique. Pour donner un exemple de relation entre les modèles BSG et de Kondo citons la relation montr\'ee par Fendley, LeSage et Saleur~\cite{Fendley:1995kj} le long de la représentation de spin $1/2$ et pour $\beta<1/\sqrt 2$~:

\begin{align}\label{eq:partition_kondo_BSG}
Z_{1/2}[(q-q^{-1})x]= \frac{Z_{BSG}(q x)+Z_{BSG}(q^{-1} x)}{Z_{BSG}(x)}
\end{align}

avec ici $x=2\pi \omega_0$ et au moins pour $q$ racine de l'unité, \cad $\beta=1/\sqrt{n}$. La fonction de partition de sine-Gordon est connue jusqu'à de larges ordres en perturbation et exactement sous la forme~\cite{Fendley:1995kj}~:


\begin{align}
Z_{BSG}(x) = 1+ \sum_{n=1}^\infty \frac{x^{2n} }{\Gamma(\beta^2)^{2n}} \sum_{{\bf m}} \prod_{i=1}^n \parent{\frac{\Gamma(m_i+\beta^2(n-i+1))}{\Gamma(m_i+\beta^2(n-i)+1)}}^2
\end{align}

avec la somme faite sur tous les ensembles (tableaux de Young) ${\bf m}=(m_1,m_2,\ldots,m_n)$ pour des entiers $m_i$ tels que $m_1 \geq m_2 \geq \ldots \geq m_n$. Il existe une méthode itérative pour calculer ces sommes ordre par ordre. La fonction de partition du modèle de Kondo dans la représentation de spin $1/2$ paraît donc calculable, au moins perturbativement, dans le régime attractif. En utilisant la BSFT de Witten, nous pensons possible d'exprimer une action effective off-shell, sachant que $\beta_\pm = (1-r^2)\lambda^\pm$ et toutes les autres fonctions bêta s'annulent. La formule habituelle de relation de l'action effective et de la fonction de partition off-shell est en théorie bosonique~\cite{Witten:1992cr,Gerasimov:2000zp,Tseytlin:1986zz,Tseytlin:2000mt}~:

\begin{align}
S[T] = (1+\beta_T \partial_T )Z[T]
\end{align}


Ici, nous aurions cependant $Z[T,r]$ avec $\beta =r$ identifiée à la distance. Et le long de champ constant, l'action $S[T,r]$ serait simplement identifi\'ee au potentiel effectif. Nous devons encore exploiter cette direction d'étude. Mais les calculs semblent à portée de main au moins dans le cas bosonique. En outre, par similitude du modèle bosonique au modèle brane-antibrane dans le régime attractif, et par comparaison au développement quadratique qu'on a obtenu, nous pourrions probablement conjecturer une forme d'action effective du système brane-antibrane séparé.



